Methods for Averaging Spectral Line Data

The ideal spectral averaging method depends on one's science goals and the available information about one's data. Including low-quality data in the average can decrease the signal-to-noise ratio (SNR), which may necessitate an optimization method or a consideration of different weighting schemes. Here, we explore a variety of spectral averaging methods. We investigate the use of three weighting schemes during averaging: weighting by the signal divided by the variance ("intensity-noise weighting"), weighting by the inverse of the variance ("noise weighting"), and uniform weighting. Whereas for intensity-noise weighting the SNR is maximized when all spectra are averaged, for noise and uniform weighting we find that averaging the 35-45% of spectra with the highest SNR results in the highest SNR average spectrum. With this intensity cutoff, the average spectrum with noise or uniform weighting has ~95% of the intensity of the spectrum created from intensity-noise weighting. We apply our spectral averaging methods to GBT Diffuse Ionized Gas (GDIGS) hydrogen radio recombination line (RRL) data to determine the ionic abundance ratio, y+, and discuss future applications of the methodology.

==> yplus.tex <==
HII - Noise &  &  &  &  &  &  &  \\
 & 1.00 & 1.08 & 461.7 & 1664 & 0.21 & 0.046 & 0.001 \\\hline
DIG - Noise &  &  &  &  &  &  &  \\
 & 1.00 & 0.45 & 245.6 & 403 & 0.26 & 0.039 & 0.002 \\
 & 1.10 & 0.37 & 180.0 & 183 & 0.47 & 0.041 & 0.002 \\
 & 1.25 & 0.31 & 130.2 & 107 & 0.41 & 0.042 & 0.002 \\
 & 1.50 & 0.24 & 92.9 & 233 & 0.40 & 0.042 & 0.003 \\
 & 1.75 & 0.21 & 160.3 & 5764 & 0.21 & 0.044 & 0.002 \\
 & 2.00 & 0.13 & 140.5 & 3859 & 0.24 & 0.049 & 0.003 \\\hline
HII - Intensity-Noise &  &  &  &  &  &  &  \\
 & 1.00 & 1.08 & 488.6 & 2208 & 0.19 & 0.046 & 0.001 \\\hline
DIG - Intensity-Noise &  &  &  &  &  &  &  \\
 & 1.00 & 0.45 & 256.1 & 403 & 0.26 & 0.040 & 0.001 \\
 & 1.10 & 0.37 & 236.8 & 1134 & 0.24 & 0.040 & 0.002 \\
 & 1.25 & 0.31 & 174.9 & 659 & 0.29 & 0.039 & 0.002 \\
 & 1.50 & 0.24 & 98.5 & 233 & 0.40 & 0.042 & 0.003 \\
 & 1.75 & 0.21 & 146.4 & 5764 & 0.21 & 0.048 & 0.002 \\
 & 2.00 & 0.13 & 133.8 & 4136 & 0.29 & 0.054 & 0.003 \\
